Enclosing Points with Geometric Objects

Let $X$ be a set of points in $\mathbb{R}^2$ and $\mathcal{O}$ be a set of geometric objects in $\mathbb{R}^2$, where $|X| + |\mathcal{O}| = n$. We study the problem of computing a minimum subset $\mathcal{O}^* \subseteq \mathcal{O}$ that encloses all points in $X$. Here a point $x \in X$ is enclosed by $\mathcal{O}^*$ if it lies in a bounded connected component of $\mathbb{R}^2 \backslash (\bigcup_{O \in \mathcal{O}^*} O)$. We propose two algorithmic frameworks to design polynomial-time approximation algorithms for the problem. The first framework is based on sparsification and min-cut, which results in $O(1)$-approximation algorithms for unit disks, unit squares, etc. The second framework is based on LP rounding, which results in an $O(\alpha(n)\log n)$-approximation algorithm for segments, where $\alpha(n)$ is the inverse Ackermann function, and an $O(\log n)$-approximation algorithm for disks.

==> conclusion.tex <==
\section{Conclusion}
%can we use planar 3-SAT?
Although many problems related to the enclosing problem have been proved to be NP-hard, the hardness status of the particular (uncolored) version \EnclosingPoints that we study here is still unknown. To complement our approximation results, it would be nice to prove that this problem is NP-hard (if that's true).
\begin{itemize}
\item Is the \EnclosingPoints problem NP-hard, e.g., when the objects are disks or arbitrary line segments in $\R^2$?
\end{itemize}

For future work on this topic, it is interesting to see whether our ideas can be extended to other geometric objects, and whether the approximation factor of our algorithms can be further improved, e.g., to near-constant. More generally, can our ideas be applied to solve other similar geometric optimization problems?

==> useless <==




\paragraph{FPT results.} These problems were also considered in the FPT context. For \ObstacleRemoval, Korman et al.\ \cite{KormanLSS18} showed that the problem is FPT for unit disks, and for similarly-sized $\beta$-fat regions with bounded ply and constant number of pairwise boundary intersections. Eiben and Kanj generalized their result to graphs satisfying the color-connectivity property \cite{EibenK18,EibenK20}. Eiben and Lokshtanov presented an FPT algorithm with $q^{O(q^3)}n^{O(1)}$ running time for general connected obtacles \cite{EibenL20}.

Kumar et al.\ \cite{0004L0S022} improved the running time for \ObstacleRemoval to $2.3146^qn^{O(1)}$, and also gave a $2^{O(p)}n^{O(k)}$-time algorithm for \GeneralizedPointsSeparation, which receives $n$ objects, a set $A$ of $k$ points, and $p$ pairs of points from $A$ as input, and asks to select the minimum number of objects to separate these pairs.

\quad

We remark that these seemingly similar problems may require different techniques to design approximation algorithms; and to the best of our knowledge, our particular version that requires enclosing all of the points (i.e., \EnclosingPoints) has not been studied before.





%\input{enclosing_points/introduction}

In this chapter, we develop approximation algorithms for the problem of enclosing all points with geometric objects (\EnclosingPoints), which is related to geometric set cover. We solve this problem by adapting techniques for approximating geometric set cover.


\paragraph{A generalized colored enclosing problem.}
To solve the \EnclosingPoints problem (Problem~\ref{prob:enclosing}), we design a polynomial-time approximation algorithm that in fact works for a generalized version of it, where each input object has a color. The goal is to ensure that each point is enclosed by a subset of the chosen objects with the same color. The colored version of the \EnclosingPoints problem is formally defined as follows:

\begin{problem}[\EnclosingPointsColored]\label{prob:enclosing_colored}
Given a set $X$ of points and a set $S$ of colored geometric objects (possibly overlapping) in $\R^2$, find the smallest subset $S^*\subseteq S$ to enclose all points in $X$. More precisely, for each point $p\in X$, there exists a subset $S_{c_p}^*\subseteq S^*$ of objects with the same color $c_p$ that encloses $p$, i.e., any curve connecting $p$ with infinity $(+\infty,0)$ must intersect at least one object in $S^*$ with color $c_p$.
\end{problem}
%Enclosing all points with colored geometric objects

The previous (uncolored) \EnclosingPoints problem (Problem~\ref{prob:enclosing}) can be viewed as a special case of the above \EnclosingPointsColored problem (Problem~\ref{prob:enclosing_colored}), since in the colored version, we can let all input objects have the same color.

\paragraph{Hardness.} It is easy to see that geometric set cover is also a special case of the above colored enclosing problem, by assigning a unique color for each object in Problem~\ref{prob:enclosing_colored}. In this way, if in the colored enclosing problem a point $p\in X$ is enclosed by objects with the same color $c_p$, then in the set cover problem, $p$ must be covered by the unique object with color $c_p$. Therefore, Problem~\ref{prob:enclosing_colored} is NP-hard for a wide range of geometric objects, e.g., unit disks or unit squares, because of the known hardness results for geometric set cover \cite{DBLP:journals/ipl/FowlerPT81}.


\subsection{Our Results}

For enclosing all points with colored geometric objects (Problem~\ref{prob:enclosing_colored}), we obtain the following results:
\begin{itemize}
\item A polynomial-time $O(\alpha(n)\log n)$-approximation algorithm for enclosing all points in $\R^2$ using colored arbitrary line segments (Theorem~\ref{thm:enclosing_segments}).
\item A polynomial-time $O(\log n)$-approximation algorithm for enclosing all points in $\R^2$ using colored disks (Theorem~\ref{thm:enclosing_disks}).
\item More generally, our results hold for curves that pairwise intersect only at most $s=O(1)$ times, achieving $O(\frac{\lambda_{s+2}(n)}{n}\log n)$-approximation (Theorem~\ref{thm:enclosing_curves}).
\end{itemize}
We remark that in particular, these results hold for the original (uncolored) \EnclosingPoints problem as a special case. To the best of our knowledge, no polynomial-time approximation algorithms were known for these problems before our work.














\section{LP-based Approximation Algorithms}
Here we present approximation algorithms for enclosing points with colored geometric objects. Our approach works for disks, arbitrary line segments, and more generally curves that pairwise intersect $O(1)$ times. In the following, we explain our approach in terms of line segments as an example.
%(or more generally objects with linear union complexity)

A common technique for designing approximation algorithms for set cover related problems is to use LP rounding. The idea is to first design and solve an LP relaxation (i.e., getting a fractional solution), and then round the LP solution to get an integral solution. Our algorithm follows this line of approach, which requires nontrivial geometric insights for designing and rounding the LP, as we will show.


\paragraph{Formulation of the LP relaxation.} We first formalize an LP relaxation of the colored enclosing problem. Intuitively, the idea is as follows: a point $q$ is enclosed by a set of line segments $S_c$ of color $c$, iff the outer boundary of these line segments enclose $q$. So it suffices to specify the outer boundary $\mathcal{B}_c$ of the union of line segments with color $c$ that we select in the solution. $\mathcal{B}_c$ is a set of disjoint simple polygons (as shown in Fig.~\ref{fig:outer_boundary_cycles}), which can also be viewed as a set of cycles on a graph $G_c$: the vertices of $G_c$ are intersection points between two line segments in $S_c$, and the edges of $G_c$ are subsegments between a pair of vertices in $G_c$ that lie on the same segment in $S_c$. To get a fractional solution, our goal is to select a set of colored fractional cycles on $G_c$ to enclose all points. We can form the constraints for each color class $c$ separately.
% (TODO: after removing the segments on the corners)

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.55\textwidth]{imgs/outer_boundary_cycles.pdf}
    \caption{The outer boundary $\mathcal{B}_c$ of the union of line segments with color $c$ is a set of disjoint simple polygons (shown in red).}
    \label{fig:outer_boundary_cycles}
\end{figure}


We now formally describe our LP. We start with specifying the variables in the LP. For each color class $c$, let $S_c$ denote the set of the input line segments with color $c$. The arrangement of $S_c$ can be viewed as a planar graph $Arr_c$, which has $O(|S_c|^2)$ vertices and edges. Each vertex in $Arr_c$ is an intersection point of two line segments in $S_c$. We then create a new graph $G_c$, using the same set of vertices as $Arr_c$. For each line segment $\ell\in S_c$, let $V(\ell)$ denote the set of all vertices in $G_c$ that lie on $\ell$. For each pair of points $u,v\in V(\ell)$, create a variable $x_{uv}^{(\ell)}$ where $0\leq x_{uv}^{(\ell)}\leq 1$, indicating the directed subsegment $uv$ of $\ell$ (with direction from $u$ to $v$) is selected $x_{uv}^{(\ell)}$ times in the fractional solution. We call $x_{uv}^{(\ell)}$ the weight of the subsegment $uv$. Also create a directed edge $e_{uv}^{(\ell)}$ from $u$ to $v$ in $G_c$.
%, and also including the two endpoints of $\ell$
%(In the special case, if $\ell$ does not intersect any other line segment, then we also create a variable $x_{00}^{(\ell)}$ to denote the whole line segment $\ell$.)

We emphasize that we need to create two variables (and respectively, two directed edges in $G_c$) for each undirected subsegment $uv$, because to ensure all points are enclosed according to the winding number constraints to be defined later, we need to know whether $uv$ appears on the boundary of the solution in clockwise or counter-clockwise order.

\quad

We next present the formulas for the constraints of our LP. There are two types of constraints that need to be handled:

1. \emph{Flow constraints.} To ensure that the solution to the LP is a set of colored fractional cycles, we design the flow constraints as follows:

For each color $c$, and for each vertex $u$ of $G_c$, we create the constraint
\[\sum_{v,\ell:~e_{uv}^{(\ell)}\in E(G_c)} x_{uv}^{(\ell)}=\sum_{v,\ell:~e_{vu}^{(\ell)}\in E(G_c)} x_{vu}^{(\ell)}.\]

The solution to the LP with respect to each color $c$ is a circulation on $G_c$. Using standard techniques, this circulation can be decompose into $O(\sum_c |E(G_c)|)=O(\sum_c |S_c|^2)=O(n^2)$ fractional cycles in polynomial time: repeatedly select the smallest variable $x_{uv}^{(\ell)}$ that is strictly positive, find a path $P_{vu}$ from $v$ to $u$ on $G_c$ using only edges with strictly positive values (such path always exists, and the value of each edge on the path is at least $x_{uv}^{(\ell)}$), and subtract the fractionally weighted cycle $\mathcal{C}$ formed by combining $e_{uv}^{(\ell)}$ and $P_{vu}$ from the solution. The fractional cycle $\mathcal{C}$ has weight $w_{\mathcal{C}}=x_{uv}^{(\ell)}$. Each round sets the value of at least one variable $x_{uv}^{(\ell)}$ to $0$, so the process will terminate in $O(|E(G_c)|)$ steps. Each cycle on $G_c$ corresponds to a monochromatic polygon with color $c$, so the LP solution can be decomposed into $O(n^2)$ fractionally weighted monochromatic polygons. We remark that these polygons are not necessarily simple.


2. \emph{Winding number constraints.} To ensure that each point in $X$ is enclosed by the outer boundary of the union of the chosen subsegments, the idea is to constrain their winding number. After orienting each (unknown) simple polygon on the outer boundary of the optimal solution $S^*$ in counter-clockwise order, the winding number of each point $q\in X$ is exactly $1$. So it suffices to ensure a similar inequality when we form the constraints for the fractional solution to the LP.

For each point $q\in X$, let $\vec{r}_q$ be an arbitrary ray starting from $q$. Inspired by the winding-number algorithm, we add the following constraint to ensure the winding number of $q$ with respect to the LP solution that we selected is at least $1$:
\[\sum_{c,\ell,u,v:~e_{uv}^{(\ell)}\text{ crosses }\vec{r}_q\text{ in counter-clockwise order}} x_{uv}^{(\ell)}-\sum_{c,\ell,u,v:~e_{uv}^{(\ell)}\text{ crosses }\vec{r}_q\text{ in clockwise order}} x_{uv}^{(\ell)}\geq 1,~\forall q\in X.\]
The (weighted) winding number of $q$ equals to the total weight of the edges that cross the ray $\vec{r}_q$ in counter-clockwise direction, minus the total weight of the edges that cross the ray $\vec{r}_q$ in clockwise direction.

We remark that we require the winding number of each point to be at least $1$ instead of exactly $1$, since in the LP solution, each polygon may not be simple, which means the winding numbers can be greater than $1$.

The winding number constraints together with the flow constraints ensure that each point is enclosed by the fractional cycles in the LP solution. Namely, for each point $p\in X$, we have
\[\sum_{\text{cycle }\mathcal{C}} w_{\mathcal{C}}\cdot \wind(q,\mathcal{C})\geq 1.\]
%3. Constraint on $x_{uv}$. For each edge $(u,v)$, we form the constraint $0\leq x_{uv}\leq 1$.

The objective function is to minimize the total weight of the (fractionally) selected subsegments:
\[\opt=\min \sum_{c,\ell,u,v:~e_{uv}^{(\ell)}\in E(G_c)} x_{uv}^{(\ell)}.\]




\paragraph{Rounding the LP.} After solving the LP to compute the optimal fractional solution in polynomial time, we represent the LP solution as a set of fractionally weighted monochromatic cycles on the disjoint union of graphs $G_c$, then rounding the fractional solution to obtain an integral solution. This is a standard technique that is commonly used for approximating set cover solutions \cite{DBLP:books/daglib/0004338}.

Here we provide a simple self-contained description, which is by using randomized rounding~\cite{RaghavanT87}. Namely, for each cycle $\mathcal{C}$ of weight $w_\mathcal{C}$, we randomly and independently select it with probability $\min\{10w_\mathcal{C}\log n,1\}$. Here selecting a cycle means selecting all subsegments contained as edges on that cycle, and if a subsegment $e_{uv}^{(\ell)}$ of an input line segment $\ell$ is selected, then the whole segment $\ell$ is included in our integral solution. Note that a line segment $\ell$ may be included because of multiple subsegments of it are selected during the rounding process; although it suffices to include $\ell$ just once, in the analysis below, we treat as if $\ell$ would be included multiple times. We show that this will not affect the approximation factor by much, because the combinatorial complexity of the outer boundary of the objects we consider is close to linear.

Our goal is to ensure all points $q\in X$ have winding number $\geq 1$ w.h.p.\ after the rounding process, which implies that they are enclosed by the integral solution, but a technical issue arises for cycles that are not simple: they may wind around a point multiple times, resulting in a large positive winding number for the point. In this case, even giving a small weight to the cycle can still ensure the (weighted) winding number of that point is at least $1$ in the fractional solution to the LP, but that means the cycle will only be selected with a small probability during the rounding process (selecting the cycle with a larger probability would be too costly).

To handle the above issue, the idea is to unwind the non-simple cycles first before rounding, i.e., decompose them into a set of simple cycles, and then randomly select each simple cycle independently. This ensures that each cycle $\mathcal{C}$ in the fractional solution contributes at most once to the winding number of any point $q$.

To unwind the non-simple cycles, we repeatedly choose a self-intersection point $v$ of the cycle $\mathcal{C}$. Suppose $v$ is the intersection point of a pair of crossing edges $u_1v_1$ and $u_2v_2$ of $\mathcal{C}$. We create a new vertex at $v$, subdivide the edge $u_1v_1$ into two edges $u_1v$ and $vv_1$, and similarly subdivide $u_2v_2$ into two edges $u_2v$ and $vv_2$. In this way, we decompose the cycle $\mathcal{C}$ into two cycles $\mathcal{C}_1$ and $\mathcal{C}_2$ by splitting at $v$. The total length of the cycles increases by $2$, since the two crossing edges are split into four edges. Recursively subdivide the cycles $\mathcal{C}_1$ and $\mathcal{C}_2$ if they are not simple. An example for the unwinding process is shown in Fig.~\ref{fig:unwinding}.
%The total running time is polynomial.
%the number of newly created arcs satisfy the recursion f(n)=f(n_1)+f(n-n_1+O(1)) for some n_1 (the length of the first cycle) => f(n)=O(n)

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.4\textwidth]{imgs/unwinding.pdf}
    \caption{During the unwinding process, the non-simple cycle $\mathcal{C}=u_1v_1w_2u_2v_2w_1$ with length 6 is decomposed into two simple cycles $\mathcal{C}_1=vv_2w_1u_1$ and $\mathcal{C}_2=vv_1w_2u_2$ each with length 4.}
    \label{fig:unwinding}
\end{figure}

To upper bound the approximation ratio, we show that it only loses a constant approximation factor at the step of decomposing non-simple cycles into simple cycles. Let $f(n)$ denote the maximum total number of edges that a non-simple cycle of length $n$ can decompose into. $f(n)$ satisfies the recurrence
\[f(n)\leq \max_{3\leq n_1\leq n-1} \left(f(n_1)+f(n-n_1+2)\right),\]
since a simple cycle formed by line segments would have length at least $3$. The edge case is $f(n)=n$ for $n\leq 3$. Solving the recurrence, we get $f(n)\leq 3n-6=O(n)$.

After decomposing the cycles into simple cycles, it still holds that for each point $q\in X$,
\begin{flalign*}
&\sum_{\text{cycle }\mathcal{C}} w_{\mathcal{C}}\cdot \wind(q,\mathcal{C})\\
&= \sum_{\text{simple cycle }\mathcal{C}} w_{\mathcal{C}}\cdot \wind(q,\mathcal{C})\\
&= \sum_{\text{simple counter-clockwise cycle }\mathcal{C}:~\mathcal{C}\text{ encloses }q} w_{\mathcal{C}}-\sum_{\text{simple clockwise cycle }\mathcal{C}:~\mathcal{C}\text{ encloses }q} w_{\mathcal{C}}\\
&\geq 1.
\end{flalign*}
We can ignore the simple cycles that appear in clockwise order, because they only contribute negatively to the winding number constraints. If we only consider the counter-clockwise cycles, it still holds that
\[\sum_{\text{simple counter-clockwise cycle }\mathcal{C}:~\mathcal{C}\text{ encloses }q} w_{\mathcal{C}}\geq 1.\]

Now we analyze the probability of failure. After the rounding process, for any $q\in X$,
\begin{flalign*}
&\Pr[q\text{ is not enclosed}]\\
&=\prod_{\text{simple counter-clockwise cycle }\mathcal{C}:~\mathcal{C}\text{ encloses }q}\Pr[\mathcal{C}\text{ is not selected}]\\
&=\prod_{\text{simple counter-clockwise cycle }\mathcal{C}:~\mathcal{C}\text{ encloses }q}\left(1-\min\{10w_{\mathcal{C}}\log n,1\}\right)\\
&\leq \lim_{k\rightarrow \infty}\left(1-\frac{10\log n}{k}\right)^{k}\\
&\leq e^{-10\log n}\leq \frac{1}{n^{10}}.
\end{flalign*}
By union bound, the probability of existing any point $q\in X$ that is not enclosed is at most
\[\Pr[\exists q\in X,~q\text{ is not enclosed}]\leq n\cdot \frac{1}{n^{10}}\leq \frac{1}{n^{9}}.\]

Therefore, the rounding process succeeds w.h.p. We remark that the approach can be derandomized, by the standard method of conditional probabilities \cite{Raghavan88}.



\paragraph{Analyzing the approximation ratio.} It is easy to see that the optimal solution $S^*$ corresponds to a feasible solution to the LP: if for each color class $c$, set the variables corresponding to the directed subsegments on the outer boundary (ordered counter-clockwise) of the line segments $S_c^*$ with color $c$ in the optimal solution to be $1$, and let all other variables being $0$, we will obtain a feasible solution to the LP. From the known combinatorial complexity of the outer face in the arrangement of line segments, the outer boundary of $S_c^*$ can be decomposed into $O(|S_c^*|\cdot \alpha(|S_c^*|))$ subsegments. Therefore the optimal LP solution satisfies
\[\opt\leq O\left(\sum_c|S_c^*|\cdot \alpha(|S_c^*|)\right)\leq O\left(|S^*|\cdot \alpha(|S^*|)\right).\]

As we have shown before, after the unwinding step, the total weight of edges among all cycles only increases by a constant factor, which is still $O(\opt)$. So after performing randomized rounding on the unwound fractional solution, the expected size of the obtained integral solution is at most
\begin{flalign*}
&\sum_{\text{simple counter-clockwise cycle }\mathcal{C}}10w_\mathcal{C}\log n \cdot O\left(|\mathcal{C}|\right)\\
&=10\log n\cdot \sum_{\text{simple counter-clockwise cycle }\mathcal{C}}\sum_{\ell,u,v:~e_{uv}^{(\ell)}\in \mathcal{C}} w_\mathcal{C}\\
&=O(\log n)\cdot \sum_{\ell,u,v}\sum_{\text{simple counter-clockwise cycle }\mathcal{C}:~\mathcal{C}\ni e_{uv}^{(\ell)}} w_\mathcal{C}\\
&\leq O(\log n)\cdot \sum_{\ell,u,v}\sum_{\text{cycle }\mathcal{C}:~\mathcal{C}\ni e_{uv}^{(\ell)}} w_\mathcal{C}\\
&\leq O(\log n)\cdot \sum_{\ell,u,v} x_{uv}^{(\ell)}\\
&\leq O(\opt\log n)\\
&\leq O\left(|S^*|\cdot \alpha(|S^*|)\log n\right).
\end{flalign*}
%if we decompose a nonsimple cycle into two, we create two more segments



\quad

In summary, the problem of enclosing points by geometric objects can be viewed as selecting the smallest subset of objects to cover all curves connecting a point $q$ with infinity (i.e.\ a set cover problem). The difficulty is there are infinitely many such curves, so directly applying the known set cover results does not give us a good approximation. Using the winding number idea, we transform the problem into covering each of a finite number of rays with a finite number of possible boundary curves of the input objects, so that we can apply the set cover approximation techniques.
%possibilities of fractional simple cycles

%\paragraph{Disks.}
%\newline
\quad

Using the above algorithm, we obtain the following approximation result for enclosing all points in $\mathbb{R}^2$ using (colored) line segments:

\begin{theorem}\label{thm:enclosing_segments}
Given a set $X$ of points and a set $S$ of colored arbitrary line segments in $\R^2$, where $|X|+|S|=n$, there exists a polynomial-time $O(\alpha(n)\log n)$-approximation algorithm for enclosing all points in $X$ using the smallest subset of objects in $S$.
\end{theorem}

\paragraph{Disks and more general types of curves.} The technique we described above can be modified to work for more general types of curves with minor changes. For curves that pairwise intersect only $s=O(1)$ times, one technical issue is during unwinding, a simple cycle may only have length $2$. If we decompose a cycle $\mathcal{C}$ into a cycle $\mathcal{C}_1$ with length $2$ and another cycle $\mathcal{C}_2$, then the length of $\mathcal{C}_2$ is the same as $\mathcal{C}$, therefore not getting a good recurrence for the maximum total size $f(n)$ of the simple cycles that we decompose into.

To fix this issue, we first try to unwind at a self-intersection point $v$ of $\mathcal{C}$, such that the two subcycles have length strictly less than $|\mathcal{C}|$. If such point exists, then our previous analysis for the recurrence of $f(n)$ still works. Otherwise if there are no such points, then it means only pairs of consecutive edges on the cycle $\mathcal{C}$ can intersect. In this case, there are only at most $s\cdot |\mathcal{C}|$ self-intersections on $\mathcal{C}$, so we can decompose $\mathcal{C}$ into $O(s|\mathcal{C}|)$ subcycles, increasing the total number of edges by only a factor of $O(s)=O(1)$.
%otherwise can unwind at another intersection point.

%Let $f(n)$ denote the maximum total number of edges that a non-simple cycle of length $n$ can decompose into. $f(n)$ satisfies the recurrence
%\[f(n)\leq \max_{2\leq n_1\leq n} \left(f(n_1)+f(n-n_1+2)\right),\]


Since it is known that the outer boundary for disks has complexity $O(n)$, we get the following result for disks:
\begin{theorem}\label{thm:enclosing_disks}
Given a set $X$ of points and a set $S$ of colored disks in $\R^2$, where $|X|+|S|=n$, there exists a polynomial-time $O(\log n)$-approximation algorithm for enclosing all points in $X$ using the smallest subset of objects in $S$.
\end{theorem}

More generally, for curves that pairwise intersect at most $s$ times, it is known that the combinatorial complexity of the outer face in the arrangement is bounded by $O(\lambda_{s+2}(n))$~\cite{DBLP:journals/dcg/GuibasSS89,AgarwalS00} as mentioned earlier in Sec.~\ref{sec:enclosing_preliminaries}. So our approximation algorithm yields the following result:
%curved segments
%(or objects with linear union complexity)
%(or polygons with constant complexity)
\begin{theorem}\label{thm:enclosing_curves}
Given a set $X$ of points and a set $S$ of colored curves that pairwise intersect at most $s=O(1)$ times in $\R^2$, where $|X|+|S|=n$, there exists a polynomial-time $O(\frac{\lambda_{s+2}(n)}{n}\log n)$-approximation algorithm for enclosing all points in $X$ using the smallest subset of objects in $S$.
\end{theorem}
